A Deployed Online Reinforcement Learning Algorithm In An Oral Health Clinical Trial

Dental disease is a prevalent chronic condition associated with substantial financial burden, personal suffering, and increased risk of systemic diseases. Despite widespread recommendations for twice-daily tooth brushing, adherence to recommended oral self-care behaviors remains sub-optimal due to factors such as forgetfulness and disengagement. To address this, we developed Oralytics, a mHealth intervention system designed to complement clinician-delivered preventative care for marginalized individuals at risk for dental disease. Oralytics incorporates an online reinforcement learning algorithm to determine optimal times to deliver intervention prompts that encourage oral self-care behaviors. We have deployed Oralytics in a registered clinical trial. The deployment required careful design to manage challenges specific to the clinical trials setting in the U.S. In this paper, we (1) highlight key design decisions of the RL algorithm that address these challenges and (2) conduct a re-sampling analysis to evaluate algorithm design decisions. A second phase (randomized control trial) of Oralytics is planned to start in spring 2025.

==> paper_outline.tex <==
\section*{Paper Outline}
\begin{enumerate}
    \item Intro \begin{itemize}
        \item Application Motivation: Dental disease, behavioral health, mobile health, need for supplement to clinician-delivered care
        \item Figure 1: Oralytics logo and toothbrush, basic Oralytics facts, num. participants, recruitment rate, population, num. of days in study, num. decision pts. per day, etc.
        \item This is a natural application for AI / RL; however, deploying AI / RL systems is challenging because of (1) and (2).
        \item In this paper, we highlight key design decisions to show how we addressed these research challenges in Oralytics.
    \end{itemize}
    \item Related Work
    \begin{itemize}
        \item Implemented online RL for optimizing message delivery in mobile health. How do we differ?
        \item \textbf{What makes Oralytics special?} Need to balance reward maximization with the ability to do a primary analysis. Everything needed to be protocolized / one way door because of the clinical trial setting.
    \end{itemize}
    \item Preliminaries \begin{itemize}
        \item Basics of Oralytics clinical trial. population, location, etc. 
        \item Basics of RL definitions, action-selection, and updating
    \end{itemize}
    \item Deploying Oralytics \begin{itemize}
        \item System design and pipeline. Maybe what a typical day looks like and weekly updates look like?
        \item (1) how we dealt with limited data. Solution examples: BLR vs. ZIP, full pooling, reward design
        \item (2) how we dealt with real-world constraints (i.e., not being able to directly access sensor data, app opening issue and dealing with anything that could go wrong like networking issues). Solution: (1) compromises in state space, (2) fallback methods.
    \end{itemize}
    \item Application Payoff
    \begin{itemize}
        \item Post-Mortem Analysis to investigate algorithm behavior. We use descriptive statistics as a tool to describe algorithm behavior. This helps with interpretability of what the algorithm did and planning for future implementations. Example our state space design, were there any covariates that didn't really matter? Ex: In a particular bin of states on average across users, did the reward and proximal outcome go up?: Look at bins for discrete state values how do the rewards look? Report on final posterior means and variance at the end of the trial and interpret what it means. Descriptive statistics to show that the algorithm is working. These statistics provide indication of something we didn't anticipate pre-deployment.
    \end{itemize}
    \item Lessons Learned \begin{itemize}
        \item Trading off bias-variance
        \item In developing AI solutions for our clinical setting, there are many technical challenges that may not need complex models. In fact, simple interpretable models in communication with domain experts is better for our setting. By taking consideration the domain and structure in the problem setting, we can improve computation (e.g., reward design).
        \item unexpected issues that we wished we could do better next time
    \end{itemize}
    \item Discussion
\end{enumerate}
